Can You Share Your Story? Modeling Clients' Metacognition and Openness for LLM Therapist Evaluation

Understanding clients' thoughts and beliefs is fundamental in counseling, yet current evaluations of LLM therapists often fail to assess this ability. Existing evaluation methods rely on client simulators that clearly disclose internal states to the therapist, making it difficult to determine whether an LLM therapist can uncover unexpressed perspectives. To address this limitation, we introduce MindVoyager, a novel evaluation framework featuring a controllable and realistic client simulator which dynamically adapts itself based on the ongoing counseling session, offering a more realistic and challenging evaluation environment. We further introduce evaluation metrics that assess the exploration ability of LLM therapists by measuring their thorough understanding of client's beliefs and thoughts.

==> latex/figures/simulated_session.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{latex/images/simulated_session.png}
    \caption{Sample figure}
    \label{fig:simulated_session}
\end{figure}

==> latex/tables/RQ4_ctrs.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{l c}
        \toprule
        \textbf{Model} & \textbf{CTRS} \\
        \midrule
        GPT-4o-mini & 5.0621 \\
        GPT-4o & 4.8844 \\
        LLaMA-3.1-70B & 5.3206 \\
        LLaMA-3.1-8B & 4.9923 \\
        Claude-3.5-Haiku & 5.6930 \\
        \textsc{Camel} & 5.0417 \\
        \bottomrule
    \end{tabular}
    \caption{CTRS scores across various models}
    \label{tab:ctrs_scores}
\end{table}

==> latex/tables/RQ4_panas.tex <==
\begin{table*}[t!]
\centering
\small
\setlength{\tabcolsep}{2pt}
\renewcommand\arraystretch{1.1}
\resizebox{\textwidth}{!}
{
\begin{tabular}{lcccccccccc}
    \toprule
    \multirow{2.5}{*}{Model} & \multicolumn{2}{c}{\textbf{Total}} & \multicolumn{2}{c}{\textbf{Easy}} & \multicolumn{2}{c}{\textbf{Normal}} & \multicolumn{2}{c}{\textbf{Hard}}\\ 
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} 
    & positive $\uparrow$ & negative $\downarrow$ & positive $\uparrow$ & negative $\downarrow$ & positive $\uparrow$ & negative $\downarrow$ & positive $\uparrow$ & negative $\downarrow$ \\
    \midrule
    \text{GPT-4o-mini}&-0.06& \textbf{+0.04} & -0.08	&\textbf{-0.53} & +0.01	&-0.02& +0.12	&+0.68 \\
    \text{GPT-4o}&-0.01&	+0.09 &+0.21	&+0.29 &-0.01&	\textbf{-0.2}& +0.05	&+0.45  \\
    \text{Llama-3.1-70B}&-0.3	&+0.11&+0.13	&+0.29& -0.51	&-0.07& 0	&+0.27   \\
    \text{Llama-3.1-8B } &\textbf{+0.07}	&-0.08 &+0.17&	-0.16 &+0.19	&-0.11 &+0.04&	+0.04  \\
    \text{Claude-3.5-Haiku} & -0.15 & +0.29 & \textbf{+0.51} & +0.47 & -0.26 &+0.23 &\textbf{+0.39}  \textbf{&-0.19}   \\
    \text{\textsc{Camel}}&-0.06&	+0.22 &-0.04&	+0.33& \textbf{+0.4}	&+0.14& -0.72&	+0.25  \\
    \bottomrule
\end{tabular}
}
\caption{Results of \textsc{MINDVOYAGER} on PANAS across various models. This table illustrates the shifts in positive and negative emotions before and after counseling sessions, categorized by the client’s openness and metacognition. (TBD)}
\vspace{-10pt}
\label{tab:panas_exp}
\end{table*}


==> latex/tables/core_beliefs.tex <==
\begin{table}[h]
\centering
\resizebox{0.48\textwidth}{!}{\begin{tabular}{ll}
\toprule
\textbf{3 major categories} & \textbf{19 fine-grained categories} \\
\midrule
\multirow{9}{*}{Helpless}   & I am incompetent.                   \\
                            & I am helpless.                      \\
                            & I am powerless, weak, vulnerable.   \\
                            & I am a victim.                      \\
                            & I am needy.                         \\
                            & I am trapped.                       \\
                            & I am out of control.                \\
                            & I am a failure, loser.              \\
                            & I am defective.                     \\
\midrule
\multirow{6}{*}{Unlovable}  & I am unlovable.                     \\
                            & I am unattractive.                  \\
                            & I am undesirable, unwanted.         \\
                            & I am bound to be rejected.          \\
                            & I am bound to be abandoned.         \\
                            & I am bound to be alone.             \\
\midrule
\multirow{4}{*}{Worthless}  & I am worthless, waste.              \\
                            & I am immoral.                       \\
                            & I am bad - dangerous, toxic, evil.  \\
                            & I don't deserve to live.            \\
\bottomrule
\end{tabular}}
\caption{The major categories and fine-grained categories of core beliefs obtained from \citet{beck2020cognitive}.}
\label{appendix:tab:fine_grained}
\end{table}

==> latex/tables/dist_meta_open.tex <==
\begin{table}[]
\small
\begin{tabular}{lll}
                  & Metacognition & Openness \\
Basic prompt      & 5.0                   & 5.0              \\
Engineered prompt & 4.28                  & 4.15            
\end{tabular}
\end{table}

==> latex/tables/rq1_overall.tex <==
\begin{table}[ht]
\centering
\setlength{\tabcolsep}{4pt}
\renewcommand\arraystretch{1.3}
\begin{tabular}{lccccc}
\hline
\multicolumn{1}{c}{\textbf{Models}} & \textbf{SIM} & \textbf{RH} & \textbf{CB} & \textbf{IB} & \textbf{CS} \\ \hline
GPT-4o-mini                         & 0.17 & 0.22 & 0.30 & 0.12 & 0.05  \\
GPT-4o                             & 0.17 & 0.24 & 0.26 & 0.13 & 0.05            \\
Llama-3.1-8B                       & 0.17 & 0.21 & 0.24 & 0.12 & 0.09             \\
Llama-3.1-70B                        & 0.18 & 0.23 & 0.28 & 0.12 & 0.10             \\
Claude-3.5-Haiku                    & 0.19 & 0.30 & 0.30 & 0.13 & 0.05             \\
CAMEL                               & 0.16 & 0.21 & 0.26 & 0.13 & 0.03             \\ \hline
\end{tabular}
\caption{Main table of RQ1}
\label{tab:rq1_overall}
\end{table}
